An Extensible Quantum Network Simulator Built on ns-3: Q2NS Design and Evaluation

As quantum networking hardware remains costly and not yet widely accessible, simulation tools are essential for the design and evaluation of quantum network architectures and protocols. However, designing a scalable and computationally efficient quantum network simulator is intrinsically challenging: i) quantum dynamics must be emulated on classical computing platforms while capturing the stateful and non-local nature of entanglement, a quantum resource without any classical networking analog; ii) quantum networking is inherently hybrid, as protocol execution also fundamentally depends on classical signaling. This makes a tight and faithful co-simulation of quantum operations and classical message exchanges a core requirement. In this light, we present Q2NS, a modular and extensible quantum network simulator, built on top of ns-3, designed to seamlessly integrate quantum-network primitives with ns-3's established classical protocol stack. Q2NS adopts a modular architecture that decouples protocol control logic from node- and channel-level operations, enabling rapid prototyping and adaptation across heterogeneous and evolving Quantum Internet scenarios. Q2NS natively supports multiple quantum state representations through a unified interface, allowing interchangeable state-vector, density-matrix, and stabilizer backends. We validate Q2NS through realistic use-case studies and comprehensive benchmarks, demonstrating superior computational efficiency over representative state-of-the-art alternatives, while preserving modeling flexibility. Finally, we provide a dedicated visualization tool that jointly captures physical and entanglement-enabled connectivity and supports entangled-state manipulations, facilitating an intuitive interpretation of entanglement dynamics and protocol behavior. Q2NS offers a flexible, open, and scalable simulation platform for advancing Quantum Internet research.

==> Tikz/Fig5_setup.tex <==
% Tikz/swap_bars_setup.tex

\makeatletter
\newcommand\resetstackedplots{%
  \pgfplots@stacked@isfirstplottrue
}
\makeatother

\definecolor{accentblue}{RGB}{0,100,145}
\definecolor{dmgreen}{RGB}{140,25,25}
\definecolor{staborange}{RGB}{170,120,0}
\definecolor{qnscolor}{RGB}{100,35,150}
\definecolor{qnslocteal}{RGB}{70,140,135}
\definecolor{softgray}{RGB}{220,220,220}
\definecolor{graygrid}{RGB}{230,230,230}
\definecolor{qnattynet-magenta}{RGB}{158, 57, 106}

\makeatletter
\@ifundefined{pgf@pattern@name@diaglines}{
  \pgfdeclarepatternformonly{diaglines}
  {\pgfqpoint{-1pt}{-1pt}}
  {\pgfqpoint{4pt}{4pt}}
  {\pgfqpoint{4pt}{4pt}}
  {
    \pgfsetlinewidth{0.4pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
    \pgfpathlineto{\pgfqpoint{4pt}{4pt}}
    \pgfusepath{stroke}
  }
}{}
\makeatother

% ---------- CSV files ----------
\def\SwapKetFile{Data/swap/swap_ket_lowconfig.csv}
\def\SwapDmFile{Data/swap/swap_dm_lowconfig.csv}
\def\SwapStabFile{Data/swap/swap_stab_lowconfig.csv}
\def\SwapQnsFile{Data/swap/swap_qns3.csv}
\def\SwapQnsLocFile{Data/swap/swap_qns3_local.csv}

% ---------- read tables ----------
\pgfplotstableread[col sep=comma]{\SwapKetFile}\swapket
\pgfplotstableread[col sep=comma]{\SwapDmFile}\swapdm
\pgfplotstableread[col sep=comma]{\SwapStabFile}\swapstab
\pgfplotstableread[col sep=comma]{\SwapQnsFile}\swapqns
\pgfplotstableread[col sep=comma]{\SwapQnsLocFile}\swapqnsloc
